Stance Detection on Social Media with Fine-Tuned Large Language Models

Stance detection, a key task in natural language processing, determines an author's viewpoint based on textual analysis. This study evaluates the evolution of stance detection methods, transitioning from early machine learning approaches to the groundbreaking BERT model, and eventually to modern Large Language Models (LLMs) such as ChatGPT, LLaMa-2, and Mistral-7B. While ChatGPT's closed-source nature and associated costs present challenges, the open-source models like LLaMa-2 and Mistral-7B offers an encouraging alternative. Initially, our research focused on fine-tuning ChatGPT, LLaMa-2, and Mistral-7B using several publicly available datasets. Subsequently, to provide a comprehensive comparison, we assess the performance of these models in zero-shot and few-shot learning scenarios. The results underscore the exceptional ability of LLMs in accurately detecting stance, with all tested models surpassing existing benchmarks. Notably, LLaMa-2 and Mistral-7B demonstrate remarkable efficiency and potential for stance detection, despite their smaller sizes compared to ChatGPT. This study emphasizes the potential of LLMs in stance detection and calls for more extensive research in this field.

==> app_method.tex <==
The LoRA method was particularly designed to emphasize the queries and values in the self-attention modules \cite{hu2021lora}. The hyperparameters for LoRA were set with a rank of 8, an \(\alpha\) of 16, and a dropout rate of 0.05. We employed a warmup strategy, utilizing 10\% of the training data. Training was set to run for three epochs with a learning rate of \(3 \times 10^{-4}\) and a batch size of 128. We trained the models with bfloat16 precision on an NVIDIA A100 GPU with 40GB. The fine-tuning of \texttt{Llama2-7b} on the SemEval-2016 dataset took approximately 20 minutes, while \texttt{Llama2-13b} took around 30 minutes.

